Frame-type Sensitive RDO Control for Content-Adaptive-encoding

Video transcoding is an increasingly important application in the streaming media industry. It has become important to investigate the optimisation of transcoder parameters for a single clip simply because of the immense number of playbacks for popular clips. In this paper, we explore the use of a canned optimiser to estimate the optimal RD tradeoff achievable for a particular clip. We show that by adjusting the Lagrange multiplier in RD optimisation on keyframes alone we can achieve more than 10$\times$ the previous BD-Rate gains possible without affecting quality for any operating point.

==> figs/dinner/snippets.tex <==

\begin{figure}[h]
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figs/dinner/a3.png}
  \caption{Current Approach}
  \label{fig:sfig2}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figs/dinner/b3.png}
  \caption{Proposed Approach}
  \label{fig:sfig1}
\end{subfigure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figs/dinner/a4.png}
  \caption{Current Bit-Allocation}
  \label{fig:sfig2}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figs/dinner/b4.png}
  \caption{Proposed Bit-Allocation}
  \label{fig:sfig1}
\end{subfigure}
\caption{Top Row: Zoomed-in View of a Block of Frame 1(KeyFrame) of AV1 with Top-level $\lambda$ modification with Modulation Type 4 of the clip DinnerSceneCropped; Bottom Row: Bit Allocation(Frame-Relative) of the same Block of the Frame.}
\label{fig:fig}
\end{figure}

